ASP modulo CSP: The clingcon system

We present the hybrid ASP solver clingcon, combining the simple modeling language and the high performance Boolean solving capacities of Answer Set Programming (ASP) with techniques for using non-Boolean constraints from the area of Constraint Programming (CP). The new clingcon system features an extended syntax supporting global constraints and optimize statements for constraint variables. The major technical innovation improves the interaction between ASP and CP solver through elaborated learning techniques based on irreducible inconsistent sets. A broad empirical evaluation shows that these techniques yield a performance improvement of an order of magnitude. To appear in Theory and Practice of Logic Programming

==> figures/0/acl/all.tex <==
\tikzstyle{square} = [draw=black, minimum width=4mm, minimum height=4mm]
\tikzstyle{named} = [draw=black, minimum width=20mm, minimum height=4mm]
\begin{tikzpicture}[remember picture]
        \footnotesize


			
			\node[name=cs] at (0mm+4*4mm,28mm) [square] {s};
			\node[name=cb] at (4mm+4*4mm,28mm) [square] {b};
			\node[name=cf] at (8mm+4*4mm,28mm) [square] {f};
			\node[name=cc] at (12mm+4*4mm,28mm) [square] {c};
			\node[name=cr] at (16mm+4*4mm,28mm) [square] {r};
			\node[name=ccr] at (20mm+4*4mm,28mm) [square] {cr};


			%packing
			\foreach \x in {238,4,4,4,109,62}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/343)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%labyrinth
			\foreach \x in {1255,16,15,15,373,31}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/1255)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}


			%incremental shed
			\foreach \x in {18,3,3,3,10,8}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/18)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%hashi
			\foreach \x in {116,10,11,10,30,25}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/116)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%hamclump
			\foreach \x in {32,6,6,6,31,12}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/32)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%quasi20
			\foreach \x in {208,26,28,26,187,30}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/481)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%weighted
			\foreach \x in {20,28,27,28,30,31}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/33)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}


			\setcounter{col}{0}
			\setcounter{row}{0}

			\node[name=packing] at (4mm,24mm+0.3mm)[named] {\emph{Packing}};
			\node[name=lab] at (4mm,20mm) [named] {\emph{Labyrinth}};
			\node[name=inc] at (4mm,16mm) [named] {\emph{Incremental Sheduling}};
			\node[name=hashi] at (4mm,12mm) [named] {\emph{HashiwoKakero}};
			\node[name=ham] at (4mm,8mm) [named] {\emph{HamiltonianCycle}};
			\node[name=quasi20] at (4mm,4mm) [named] {\emph{Quasi Group}};
			\node[name=weighted] at (4mm,0mm) [named] {\emph{Weighted Assignment Tree}};
%
%
  \end{tikzpicture}




==> figures/0/calls/all.tex <==
\tikzstyle{square} = [draw=black, minimum width=4mm, minimum height=4mm]
\tikzstyle{named} = [draw=black, minimum width=20mm, minimum height=4mm]
\begin{tikzpicture}[remember picture]
        \footnotesize


			
			\node[name=cs] at (0mm+4*4mm,28mm) [square] {s};
			\node[name=cb] at (4mm+4*4mm,28mm) [square] {b};
			\node[name=cf] at (8mm+4*4mm,28mm) [square] {f};
			\node[name=cc] at (12mm+4*4mm,28mm) [square] {c};
			\node[name=cr] at (16mm+4*4mm,28mm) [square] {r};
			\node[name=ccr] at (20mm+4*4mm,28mm) [square] {cr};


			%packing
			\foreach \x in {93,8,7,8,30,16}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/4159)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%labyrinth
			\foreach \x in {924,25,27,24,1133,223}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/2474)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}


			%incremental shed
			\foreach \x in {2834,67,67,73,776,234}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/8773)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%hashi
			\foreach \x in {6135,2,2,2,4472,190}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/11465)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%hamclump
			\foreach \x in {548,5,8,5,282,9}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/2310)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%quasi20
			\foreach \x in {127,1,1,4,110,2}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/1917)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%weighted
			\foreach \x in {203,105,109,87,263,223}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/2997)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}


			\setcounter{col}{0}
			\setcounter{row}{0}

      \node[name=packing] at (4mm,24mm+0.3mm)[named] {\emph{Packing}};
      \node[name=lab] at (4mm,20mm) [named] {\emph{Labyrinth}};
      \node[name=inc] at (4mm,16mm) [named] {\emph{Incremental Sheduling}};
      \node[name=hashi] at (4mm,12mm) [named] {\emph{HashiwoKakero}};
      \node[name=ham] at (4mm,8mm) [named] {\emph{HamiltonianCycle}};
      \node[name=quasi20] at (4mm,4mm) [named] {\emph{Quasi Group}};
      \node[name=weighted] at (4mm,0mm) [named] {\emph{Weighted Assignment Tree}};

%
%
  \end{tikzpicture}




==> figures/0/conflicts/all.tex <==
\tikzstyle{square} = [draw=black, minimum width=4mm, minimum height=4mm]
\tikzstyle{named} = [draw=black, minimum width=20mm, minimum height=4mm]
\begin{tikzpicture}[remember picture]
        \footnotesize


			
			\node[name=cs] at (0mm+4*4mm,28mm) [square] {s};
			\node[name=cb] at (4mm+4*4mm,28mm) [square] {b};
			\node[name=cf] at (8mm+4*4mm,28mm) [square] {f};
			\node[name=cc] at (12mm+4*4mm,28mm) [square] {c};
			\node[name=cr] at (16mm+4*4mm,28mm) [square] {r};
			\node[name=ccr] at (20mm+4*4mm,28mm) [square] {cr};


			%packing
			\foreach \x in {824,86,74,88,277,156}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/12735)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%labyrinth
			\foreach \x in {925,305,361,282,1159,679}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/2575)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}


			%incremental shed
			\foreach \x in {2521,57,60,65,599,185}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/3768)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%hashi
			\foreach \x in {8243,202,198,201,4684,450}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/11590)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%hamclump
			\foreach \x in {523,2,3,2,288,19}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/2109)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%quasi20
			\foreach \x in {1024,258,424,327,880,234}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/2827)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%weighted
			\foreach \x in {2598,3420,3775,2751,6097,5418}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/12506)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}


			\setcounter{col}{0}
			\setcounter{row}{0}

      \node[name=packing] at (4mm,24mm+0.3mm)[named] {\emph{Packing}};
      \node[name=lab] at (4mm,20mm) [named] {\emph{Labyrinth}};
      \node[name=inc] at (4mm,16mm) [named] {\emph{Incremental Sheduling}};
      \node[name=hashi] at (4mm,12mm) [named] {\emph{HashiwoKakero}};
      \node[name=ham] at (4mm,8mm) [named] {\emph{HamiltonianCycle}};
      \node[name=quasi20] at (4mm,4mm) [named] {\emph{Quasi Group}};
      \node[name=weighted] at (4mm,0mm) [named] {\emph{Weighted Assignment Tree}};

%
%
  \end{tikzpicture}




==> figures/0/time/all.tex <==
\tikzstyle{square} = [draw=black, minimum width=4mm, minimum height=4mm]
\tikzstyle{named} = [draw=black, minimum width=20mm, minimum height=4mm]
\begin{tikzpicture}[remember picture]
        \footnotesize


			
			\node[name=cs] at (0mm+4*4mm,28mm) [square] {s};
			\node[name=cb] at (4mm+4*4mm,28mm) [square] {b};
			\node[name=cf] at (8mm+4*4mm,28mm) [square] {f};
			\node[name=cc] at (12mm+4*4mm,28mm) [square] {c};
			\node[name=cr] at (16mm+4*4mm,28mm) [square] {r};
			\node[name=ccr] at (20mm+4*4mm,28mm) [square] {cr};


			%packing
			\foreach \x in {900,578,671,593,718,658}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/900)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%labyrinth
			\foreach \x in {871,133,202,114,878,742}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/896)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}


			%incremental shed
			\foreach \x in {105,12,14,16,47,17}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/123)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%hashi
			\foreach \x in {461,15,18,16,351,127}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/682)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%hamclump
			\foreach \x in {338,1,3,1,248,23}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/417)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%quasi20
			\foreach \x in {378,19,29,21,469,13}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/789)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}

			%weighted
			\foreach \x in {628,544,519,553,426,427}
			{
			%\pgfmathparse{round((\x/32)*100)} 
			\pgfmathparse{round((\x/633)*100)} 
			\setcounter{result}{\pgfmathresult}
			\pgfmathparse{(\value{col}*1.4mm)+1.4mm*4}
			\setlength{\coll}{\pgfmathresult mm}
			\pgfmathparse{(6-\value{row})*1.4mm}
			\setlength{\rowl}{\pgfmathresult mm}

			
			%\node[name=s\x] at (\value{col}/7,\pgfmathresult) [square, fill=yellow!15] {{$\arabic{col} and \pgfmathresult$}};
			%\node[name=s\x] at (\value{col},5-\value{row}) [square, fill=black!\theresult] {{\the\rowl}};
			\node[name=s\the\coll\the\rowl] at (\the\coll,\the\rowl) [square, fill=black!\theresult] {{}};
			\ifnum\value{col}=5
						\setcounter{col}{0}
						\addtocounter{row}{1}
		  \else
						\addtocounter{col}{1}
			\fi
			}


			\setcounter{col}{0}
			\setcounter{row}{0}

      \node[name=packing] at (4mm,24mm+0.3mm)[named] {\emph{Packing}};
      \node[name=lab] at (4mm,20mm) [named] {\emph{Labyrinth}};
      \node[name=inc] at (4mm,16mm) [named] {\emph{Incremental Sheduling}};
      \node[name=hashi] at (4mm,12mm) [named] {\emph{HashiwoKakero}};
      \node[name=ham] at (4mm,8mm) [named] {\emph{HamiltonianCycle}};
      \node[name=quasi20] at (4mm,4mm) [named] {\emph{Quasi Group}};
      \node[name=weighted] at (4mm,0mm) [named] {\emph{Weighted Assignment Tree}};

%
%
  \end{tikzpicture}



